Wall-crossing structures on surfaces

Families of Bridgeland stability conditions induce families of stability data, wall-crossing structures and scattering diagrams on the motivic Hall algebra. These structures can be transferred to the quantum torus if the stability conditions of the family have global dimension at most 2. We show that geometric stability conditions on surfaces with nef anticanonical bundle have global dimension 2 and we study the resulting family of stability data. We formulate a conjecture relating this family to the family of stability data associated with a quiver with potential and we verify this conjecture for the projective plane.

==> commands.tex <==
\RequirePackage{amsmath,amssymb}%,amsthm}
\RequirePackage{etoolbox,bbm,xspace}
\RequirePackage{version,xparse}
%\RequirePackage[a4paper,margin=1.35in]{geometry}

%%%% Theorem environments
\ifx\notheorems\undefined
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}{Conjecture}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\theoremstyle{remark}
\newtheorem{rmr}[theorem]{Remark}
%\newtheorem{question}[theorem]{Question}
%\AtEndEnvironment{remark}{\hfill$\lozenge$}
%\AtEndEnvironment{example}{\hfill$\lozenge$}
\fi

%%%% Auxiliary commands
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}
\def\redef#1{\csletcs{t@#1}{#1}\csdmat{#1}{\csuse{t@#1}}}
\def\opr#1#2{\dmat#1{\operatorname{#2}}}
\def\opra#1#2{\csdmat{#1}{\operatorname{#2}}}
\def\oper#1{\csdmat{#1}{\operatorname{#1}}}
\def\DMO{\opr}
\makeatletter
\def\forlist#1#2{\@xp\forcsvlist\@xp{\@xp#1\@xp}\@xp{#2}}
% usage: \forlist\command\list
\makeatother

%%%% Operators. Usage: \GL
\forcsvlist\oper{
Vect,Mod,Rep,Ab,Grp,Com,Set,Top,Sch,Coh,Qcoh,Ob,Ring,Alg,
Map,Hom,End,Aut,Ext,Cat,Sh,Ind,RHom,Fun,Var,rad,
Ker,Im,deg,Tr,det,rk,diag,im,coker,tr,cone,add,
sk,cosk,colim,Res,Gal,Coker,dlog,
GL,SL,PGL,Gr,Lib,Conv,Sol,Tor,
Max,Spec,Ass,Ann,Quot,Pic,Sym,MHS,MHM,
td,ch,Supp,supp,vol,trdeg,lc,NS,Loc,Iso,per,gr,Der,Lie,
Log,Exp,Pow,ord,lcm,VB,Hilb,cl,SU,SO,Ad,ad,id}
\opr\Id{id}
\opr\lHom{\lb{Hom}}
\opr\lAut{\lb{Aut}}
\opr\lIso{\lb{Isom}}
\opr\hgt{ht}
\opr\chr{char}
\opr\udim{\mathbf{dim}}
\opr\cls{\mathsf{cl}}
\opr\mmod{mod}
\opr\Et{\mathsf{Et}}
\def\gl{\mathfrak{gl}}
\def\sl{\mathfrak{sl}}
\def\su{\mathfrak{su}}
\def\so{\mathfrak{so}}
\oper{sgn}\def\sign{\sgn}


%%%% Symbols
\def\mto{\mapsto}
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\xlto{\xleftarrow}
\def\emb{\hookrightarrow}
\def\lemb{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\def\isoto{\xto{\,\smash{ 
	\raisebox{-3pt}{\ensuremath{\scriptstyle\sim}}
}\,}}
\dmat\es{\varnothing}%{\emptyset}
\def\bs{\backslash}
\def\sbs{\subset}
\def\sps{\supset}
\redef{iff}
\dmat\imp{\implies}
\dmat\xx{\times}
\dmat\dd{\partial}
\def\pd#1{\frac\dd{\dd#1}}
\def\iso{\simeq}
\def\ms{\backslash}
\def\bi{\mathbf i}
\def\bop{\bigoplus}
\def\ilim{\varprojlim} %inverse limit
\def\dlim{\varinjlim} %direct limit
\def\ts{\otimes}
\def\bts{\bigotimes}
\def\lb{\underline}
\def\ub{\overline}
\def\ubar#1{\mkern1.5mu\overline%
	{\mkern-1.5mu#1\mkern-1.5mu}\mkern1.5mu}
\def\oh{{\frac12}}
\dmat\Gm{\mathbb G_{\mathrm m}}
\dmat\one{\mathbbm1}
\def\qt{\delimiter"502F30E\mathopen{}} %/correct spacing
\def\dlim{\varinjlim} %direct limit
\def\ilim{\varprojlim} %inverse limit
\def\partof{\vdash}
\def\what{\widehat}
\def\tl{\tilde}
\def\wtl{\widetilde}
\def\inv{^{-1}}
\def\dual{^{\vee}}
\def\trp{^{\mathsf T}} %transpose
\dmat\pt{\mathbf{pt}}
\def\op{\mathrm{op}}
\def\st{\mathrm{s}}
\def\sst{\mathrm{ss}}
\def\nil{\mathsf {nil}}
\def\et{\mathrm{et}}
\def\ri{\mathrm i}
\def\sep{\mathrm{sep}}
\def\ab{\mathrm{ab}}
\def\top{\mathrm{top}}
\def\Ta{T^{\mathrm a}} %tensor algebra
\def\Tc{T^{\mathrm c}} %tensor coalgebra
\dmat\bul{\bullet}
\newdimen\bulh\settoheight\bulh{\bul}
\def\sbul{{\hspace{.5pt}\raisebox{.5\bulh}{%
	\scalebox{.5}{\raisebox{-.5\bulh}{\bul}}%
}}}%small bullet
\def\GIT{/\!\!/}
\def\git{\GIT}
\def\qbinom{\genfrac{[}{]}{0pt}{}}
\def\ac{{\tiny\raisebox{2pt}{\textup{!`}}}}%anti-shriek
\newlength{\mylength}

\def\xmto#1{\,\tikz{
	\settowidth{\mylength}{\mat{#1}}
	\draw(0,1mm)--(0,-1mm);
	\draw[->](0,0)--(2\mylength,0)
	node[above,midway]{\mat{#1}};
	}\,}
\def\upc{\tikz{\draw[->,>=latex'](0,0)--(0,.3)}}
%requires \usetikzlibrary{arrows}
\def\upc#1{\left\uparrow#1\right.}%upper closure
\def\loc#1{\left\downarrow#1\right.}%lower closure


%%%% Aphabets: \bA,\cA,\fA,\bfA,\sA
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\def\deffrak#1{\csdmat{f#1}{\mathfrak{#1}}}
\def\defbf#1{\csdmat{bf#1}{\mathbf{#1}}}
\def\defsf#1{\csdmat{s#1}{\mathsf{#1}}}
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}\defbf{#1}\defsf{#1}}
\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}
\def\defbl#1{\csdmat{b#1}{\mathbf{#1}}} %lower case
\forcsvlist\defbl{a,b,c,d,e,g,h,i,j,k,l,n,o,p,q,r,s,t,u,v,w,x,y,z}
%\dmat\bk{\mathbbm k}
\dmat\bk{\Bbbk}

%%%% Greek letters
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\la\lambda
\dmat\ta\tau
\dmat\hi\chi
\dmat\eps\varepsilon
\dmat\vi\phi
\dmat\te\theta
\dmat\ksi\xi
\dmat\si\sigma
\dmat\om\omega
\dmat\Ga\Gamma
\dmat\La\Lambda
\dmat\De\Delta
\dmat\Om\Omega
\dmat\Si{\Sigma}
\dmat\ze\zeta
\dmat\Te{\Theta}
\dmat\Na{\nabla}
\dmat\kp{\kappa}
\forcsvlist\redef{Phi,Psi,pi,mu,nu}
\dmat\io{\iota}

%%%% Structures
\def\set#1{\mat{\left\{#1\right\}}}
\def\sets#1#2{\left\{\left.#1\ \right\vert#2\right\}}
\def\ang#1{\mat{\left\langle#1\right\rangle}}
\def\angs#1#2{\ang{#1\col#2}}
\def\rbr#1{\left(#1\right)}
\def\sbr#1{\left[#1\right]}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\n#1{\left\lvert#1\right\rvert}
\def\nn#1{\left\lVert#1\right\rVert}
\def\eq#1{\begin{equation}#1\end{equation}}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{(\;\!\!\!(#1)\!\!\!\;)} %formal Laurent series ((#1))
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\vmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\smat#1{\left(\begin{smallmatrix}#1\end{smallmatrix}\right)}
\def\matr#1{\begin{matrix}#1\end{matrix}}
\def\pmatv#1#2{\left(\matr{#1}
	\hspace{.5ex}\middle|\hspace{.3ex}
	\matr{#2}\right)}
%\def\matr{\pmat}
\def\nop#1{\left.\col#1\col\right.}%normal oper product


%%%% Problems and solutions
%\newtheoremstyle{problem}{}{}{}{}\bf:{.5em}{}
%%%%\newtheoremstyle{problem}{}{}\em{}\bf:{.5em}{}
%\theoremstyle{problem}
%\newtheorem{prob}{Problem}
%\newif\ifsol
%\excludeversion{sol}
%\def\showsol{\soltrue%
%	\renewenvironment{sol}{\noindent{\bf Solution:}} {\hfill\qed}
%}

%%%% Diff
\def\br{\ \vspace{-.5ex}} %break after itemize
\def\dir#1#2{\noindent\textbf{(#1)$\implies$(#2).}}
\def\clm#1{\noindent\textbf{(#1)}\xspace} %claim, \cl should be used for classes
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\qq#1{\lqq#1\rqq}
\def\tpdf{\texorpdfstring} %hyperref
\def\hl{\noindent\rule{\textwidth}{1pt}}

%%%% Words and phrases
\def\ie{i.e.\@\xspace} %id est
\def\cf{cf.\@\xspace} %confer
\def\eg{e.g.\@\xspace} %exempli gratia
\def\lci{l.c.i.\@\xspace}
%\def\fd{f.d.\@\xspace} % used for \mathfrak{d}
\def\etale{\'etale\xspace}
\def\qis{quism\xspace} %quasi-isomorphism
\def\wrt{with respect to\xspace}
\def\hint{\noindent\textbf{Hint:}\xspace}
\def\Wlog{Without loss of generality\xspace}
\def\tfae{the following are equivalent\xspace}
\def\nbd{neighborhood\xspace}

%%%% Citations
\def\defcite#1#2{%\defcite\moz{mozgovoy_DT}
	\DeclareDocumentCommand{#1}{o}
		{\IfValueTF{##1}{\cite[##1]{#2}}{\cite{#2}}\xspace}
}

%%%% Colons
%\RequirePackage{mathtools}
%\mathtoolsset{centercolon} %now : is math active
%\edef\col{\mathchar\the\mathcode`:} %alternative :
%\DeclareMathSymbol\col\mathrel{operators}{"3A}
%\edef\latexequal{\mathchar\the\mathcode`=}
\mathchardef\col=\mathcode`:
\mathchardef\latexequal=\mathcode`=
\patchcmd\colon{:}{\col}{}{} %avoid the usage of :
\def\rcol{\col}

\makeatletter
{\catcode`:=\active
\gdef:{\@ifnextchar=\col\colon}}
{\catcode`==\active
\gdef={\latexequal\@ifnextchar:{\col\let\next}{}}}
\makeatother
\AtBeginDocument{\mathcode`:="8000}
\AtBeginDocument{\mathcode`=="8000}


%%%% Indexed definition \idef{name}{optional name}
\DeclareDocumentCommand{\idef}{mo}{%
	\ifmmode#1\else\textit{#1}\fi%
	\IfValueTF{#2}{\index{#2}}{\index{#1}}%
}
%\def\itodo#1{\marginnote{\bf#1}}
%%\def\itodo{\todo[color=none,bordercolor=none]}
%\def\idef#1{\ifmmode\vadjust{\itodo{$#1$}}{#1}%
%\else\itodo{#1}\textbf{#1}\fi}

%%%% Table of contents style
%\makeatletter
%\renewcommand{\tocsubsection}[3]{%
%  \indentlabel{\@ifnotempty{#2}{
%  	\hspace*{1.1em}
%  	\makebox[2.3em][l]{\ignorespaces#1 #2.\hfill}
%	}}#3\dotfill}
%\makeatother


%%% Notes
\RequirePackage[framemethod=TikZ]{mdframed}

\newmdtheoremenv[backgroundcolor=green!15,roundcorner=5pt,innertopmargin=-2.5pt,linewidth=0]{innerNote}{Note}
%\newenvironment{notes}{\begin{innerNote}}{\end{innerNote}}

\newmdtheoremenv[backgroundcolor=yellow!15,
	innertopmargin=-2pt]{innerOld}{Old material}
\newenvironment{old}{\begin{innerOld}}{\end{innderOld}}

\newenvironment{comm}[1][brown!10]
{\begin{mdframed}[backgroundcolor=#1,linewidth=0]}
{\end{mdframed}}

\def\note#1{\comm#1\endcomm}

%\newtheorem{innerNote}{Note}
\newenvironment{notes}
	{\begin{mdframed}[backgroundcolor=green!15,
		roundcorner=5pt,innertopmargin=-2.5pt,linewidth=0]
		\innerNote
	}{\endinnerNote\end{mdframed}}

%\def\note#1{\par\noindent%
%	\colorbox{yellow!15}{\textbf{Note:} #1}}

%\RequirePackage{todonotes}
%\def\note#1{\
%	\todo[size=\normalsize,inline,bordercolor=yellow,
%	backgroundcolor=yellow!15]{#1}}

%\newenvironment{note}[1][yellow!15]
%{\begin{mdframed}[backgroundcolor=#1,linewidth=0]}
%{\end{mdframed}}

%\excludeversion{notes}
%\excludeversion{comm}
%\excludeversion{old}
%\def\note#1{}

%custom number side in equations, manual number: \tag{name}
\makeatletter
\def\leqnomode{\tagsleft@true\let\veqno\@@leqno}
\def\reqnomode{\tagsleft@false\let\veqno\@@eqno}
\makeatother

%%%%% Tikz commands
\newenvironment{ctikzcd}
	{\center\tikzcd}{\endtikzcd\endcenter}
\newenvironment{ctikz}
	{\center\tikzpicture}{\endtikzpicture\endcenter}

%custom theorem, can be used to list axioms (with labels)
\theoremstyle{plain}
\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\def\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\DeclareDocumentCommand\sec{o}{
	\IfValueTF{#1}{\subsection{#1}}
			{\subsection{}\hspace{-1ex}}}

